LMap: Shape-Preserving Local Mappings for Biomedical Visualization

Visualization of medical organs and biological structures is a challenging task because of their complex geometry and the resultant occlusions. Global spherical and planar mapping techniques simplify the complex geometry and resolve the occlusions to aid in visualization. However, while resolving the occlusions these techniques do not preserve the geometric context, making them less suitable for mission-critical biomedical visualization tasks. In this paper, we present a shape-preserving local mapping technique for resolving occlusions locally while preserving the overall geometric context. More specifically, we present a novel visualization algorithm, LMap, for conformally parameterizing and deforming a selected local region-of-interest (ROI) on an arbitrary surface. The resultant shape-preserving local mappings help to visualize complex surfaces while preserving the overall geometric context. The algorithm is based on the robust and efficient extrinsic Ricci flow technique, and uses the dynamic Ricci flow algorithm to guarantee the existence of a local map for a selected ROI on an arbitrary surface. We show the effectiveness and efficacy of our method in three challenging use cases: (1) multimodal brain visualization, (2) optimal coverage of virtual colonoscopy centerline flythrough, and (3) molecular surface visualization.

==> conformal_geometry.tex <==
\section{Theoretical Background} \label{conformal_mapping}

This section introduces the basic concepts and theorems for surface Ricci flow. We refer readers to \cite{ricci2013} for details.

\subsection{Riemannian Metric}

Suppose $S$ is a surface embedded in the three dimensional Euclidean space $\mathbb{R}^3$. We select a local parameter $(u,v)$, the position vector of the surface is denoted as $\mathbf{r}:S\to\mathbb{R}^3$. The Riemannian metric defines an inner product on each tangent plane of the surface: given two tangent vectors
\[
    d\mathbf{r} = \mathbf{r}_u du + \mathbf{r}_v dv, 
    \delta\mathbf{r} = \mathbf{r}_u \delta u + \mathbf{r}_v \delta v,
\]
the inner product in $\mathbb{R}^3$ is given by 
\[
    \langle d\mathbf{r} , \delta \mathbf{r} \rangle = \begin{pmatrix} du & dv \end{pmatrix}
    \begin{pmatrix} 
    \langle \mathbf{r}_u, \mathbf{r}_u \rangle & \langle \mathbf{r}_u, \mathbf{r}_v \rangle\\
    \langle \mathbf{r}_v, \mathbf{r}_u \rangle & \langle \mathbf{r}_v, \mathbf{r}_v \rangle\\
    \end{pmatrix} 
    \begin{pmatrix}\delta u \\ \delta v \end{pmatrix}
\]
The Riemannian metric tensor is generally denoted as $\mathbf{g}$. 

For any point $p\in S$, there is a neighborhood $U(p)$, in which one can find the \emph{isothermal coordinates} $(u,v)$, such that 
\[
    \mathbf{g} = e^{2\lambda(u,v)} (du^2 + dv^2).
\] 
\subsection{Gaussian Curvature}

Suppose the surface $S$ is embedded in the Euclidean space $\mathbb{R}^3$, the normal vector is denoted as $\mathbf{n}$. The Gauss map maps each point to its normal on the unit sphere, $G: S\to \mathbb{S}^2$, $\mathbf{r}(u,v)\to \mathbf{n}(u,v)$. The Weingarten map is the derivative map of the Gauss map, $W: T_pS\to T_{\mathbf{n}(p)}\mathbb{S}^2$, $d\mathbf{r}(u,v)\to d\mathbf{n}(u,v)$. The determinant of the Weingarten map is the \emph{Gaussian curvature}.

Under the isothermal coordinates $(u,v)$, the Gaussian curvature can be calculated as 
\[
    K(x,y) = -\Delta_{\mathbf{g}} \lambda(u,v) = -\frac{1}{e^{2\lambda(u,v)}} \Delta \lambda(u,v),
\]
where $\Delta$ is the Laplace operator $\Delta = \frac{\partial^2}{\partial u^2}+\frac{\partial^2}{\partial v^2}$. 

Furthermore, according to Gauss-Bonnet theorem, the total Gaussian curvature is a topological invariant,
\begin{equation}
    \int_S K(u,v) dA_{\mathbf{g}} = \int_S K(u,v) e^{2\lambda(u,v)} dudv = 2\pi \chi(S),
    \label{eqn:Gauss_Bonnet}
\end{equation}
where $\chi(S)$ is the Euler characteristic number of the surface.

\subsection{Conformal Mapping}

Given two Riemannian surfaces $(S,\mathbf{g})$ and $(D,\mathbf{h})$, with local coordinates $(x,y)$ and $(u,v)$ respectively. The metric tensors have local representations
\[
    \mathbf{g} = 
    \begin{pmatrix} 
    g_{11} & g_{12}\\
    g_{21} & g_{22}
    \end{pmatrix},~~~
    \mathbf{h} =
    \begin{pmatrix}
    h_{11} & h_{12}\\
    h_{21} & h_{22}
    \end{pmatrix}
\]
A differential mapping $\varphi: S\to D$ has local representation $\varphi:(x,y)\mapsto (u,v)$, and induces tangential mapping $d\varphi: T_pS\to D_{\varphi(p)}$, $d\varphi: (dx,dy)\mapsto (du,dv)$. The pull-back metric is defined as
\[
    \langle d\mathbf{r}, \delta \mathbf{r} \rangle_{\varphi^*\mathbf{h}} = \langle d\varphi(d\mathbf{r}), d\varphi(\delta\mathbf{r})\rangle_{\mathbf{h}}
\]
The local representation of the pull-back metric is 
\[
    \varphi^* \mathbf{h} = 
    \begin{pmatrix}
    u_x & v_x \\
    u_y & v_y 
    \end{pmatrix} 
    \begin{pmatrix}
    h_{11} & h_{12} \\
    h_{21} & h_{22}
    \end{pmatrix}
    \begin{pmatrix}
    u_x & u_y \\
    v_x & v_y
    \end{pmatrix}.    
\]
We can define conformal mapping using pull-back metric.

\begin{definition}[Conformal Mapping]Given two Riemannian surfaces $(S,\mathbf{g})$ and $(T,\mathbf{h})$, a smooth mapping $\varphi:S\to T$ is called \emph{conformal}, if the pull-back metric induced by $\varphi$ and the original metric differ by a scalar function:    $\varphi^*\mathbf{h} = e^{2u}\mathbf{g}$,
where $u: S\to\mathbb{R}$ is a scalar function.
\end{definition}

Intuitively, conformal mapping preserves angles and maps infinitesimal circles to infinitesimal circles. Locally, a conformal map can be treated as a scaling map, then the scaling factor varies from point to point. Therefore, a conformal map preserves angles and local shapes. The shape-preserving property is crucial for visualization purposes.

\subsection{Ricci Flow}
Furthermore, given an arbitrary target Gaussian curvature $\bar{K}:S\to\mathbb{R}$, satisfying the Gauss-Bonnet condition (Eqn.~\ref{eqn:Gauss_Bonnet}), there exists a Riemannian metric $\mathbf{\bar{g}} = e^{2\lambda} \mathbf{g}$, which induces the target curvature, where $\lambda:S\to\mathbb{R}$ satisfies the Yamabe equation
\[
    \bar{K} = e^{-2\lambda}(K - \Delta_{\mathbf{g}} \lambda ),
\]
where $\Delta_{\mathbf{g}}$ is the Laplace-Beltrami operator induced by the original metric $\mathbf{g}$.

In practice, Hamilton's Ricci flow is a powerful tool to solve Yamabe equation, and to design a Riemannian metric by prescribing the target curvature.

\begin{definition}[Hamilton's Ricci Flow] Given a closed Riemannian surface $(S,\mathbf{g})$, the normalized Ricci flow is defined as
\begin{equation}
    \frac{dg_{ij}}{dt} = 2\left(\frac{2\pi\chi(S)}{A(0)}-K\right)g_{ij},
    \label{eqn:smooth_ricci_flow}
\end{equation}
where $\chi(S)$ is the Euler characteristic number of the surface, $A(0)$ is the initial total area.
\end{definition}

Hamilton and Chow proved that the surface Ricci flow converges to the constant curvature metric. In practice, we use Ricci flow to find the desired metric which induces the target curvature, 
\begin{equation}
    \frac{dg_{ij}}{dt} = 2\left(\bar{K}-K\right)g_{ij},
    \label{eqn:ricci_flow}
\end{equation}
